DenseTact 2.0: Optical Tactile Sensor for Shape and Force Reconstruction

Collaborative robots stand to have an immense impact on both human welfare in domestic service applications and industrial superiority in advanced manufacturing with dexterous assembly. The outstanding challenge is providing robotic fingertips with a physical design that makes them adept at performing dexterous tasks that require high-resolution, calibrated shape reconstruction and force sensing. In this work, we present DenseTact 2.0, an optical-tactile sensor capable of visualizing the deformed surface of a soft fingertip and using that image in a neural network to perform both calibrated shape reconstruction and 6-axis wrench estimation. We demonstrate the sensor accuracy of 0.3633mm per pixel for shape reconstruction, 0.410N for forces, 0.387Nmm for torques, and the ability to calibrate new fingers through transfer learning, which achieves comparable performance with only 12% of the non-transfer learning dataset size.

==> drafts/intro_draft_1.tex <==
\section{INTRODUCTION}


The ability for robots to perform complex dexterous manipulation is inherently dependent on the quality of the tactile sensors.

% Consider merging these two paragraphs to save space

%Tactile sensing ability for robots 
The tactile sensor's resolution, noise, bias, and repeatability all contribute directly to the robot's ability to perform robust object manipulation and control. A variety of tactile sensors have been developed with many different approaches including piezoelectric \cite{wettels2009multi}, optics \cite{Dong2017}, resistance \cite{cheng2009flexible}, magnetic\cite{yan2021soft}, or capacity. 
Recently, vision-based tactile sensors have been become very popular compared to previous sensors due to their higher resolution. Optical sensors have proven valuable for tactile sensing with usefulness in detecting both shear and normal forces \cite{Ma2019}, \textcolor{red}{controlling grasping motion \cite{}}, or adjusting grasp \cite{Hogan2018}. 


Like a human finger, tactile sensing with high resolution for robotic systems is one of the major challenges to improve dexterity of the robots. A tactile sensor that requires high resolution with versatile shape has been considered as a solution for manipulation with complexity. Recently, tactile sensors have been developed using hall effect \cite{yan2021soft}, capacity \cite{Huh2020}, or optics \cite{Dong2017} to improve the resolution and capabilities of robot manipulation. Vision-based tactile sensors have been proved valuable for multiple complex challenges such as grasping \cite{doi:10.1177/02783649211027233, Hogan2018}. The key challenge of the vision-based tactile sensor is improvements on dexterity with localization and force. Tactile sensors have been focused on increasing their capacity to detect as much information from single sensory input through soft tactile contact. Table \ref{table:comparison} compares the resolution of vision-based sensor , design shape, and force sensing modality with the range of the proposed sensor of this work in the final row.

\textcolor{red}{Among the soft tactile sensing, the major hurdle for the }
\begin{figure}[t!]
	\centering
	\includegraphics[width=2.7in]{figures/main_v2.png}
  \caption{\textbf{DenseTact 2.0.} Sensor is outfitted on the Allegro\texttrademark{} hand. Left bottom image shows the image taken from the cameras. Middle bottom shows the resultant depth image. Right bottom represents the 3D reconstructed surface of the current sensor.}
  	\label{fig:main}
      \vspace{-0.67cm}
\end{figure}
\subsection {Advantage of Non-Structural Model with High Durability} 
\textcolor{red}{We need to focus on super-soft gel force prediction}

The previous model could not resolve the nonlinearity problem on building a force estimation model. For example, Gelslim built an iFEM model, but it only works with small depth. 

Our sensor aims to solve the force estimation problem from the input as the image is detected from the super-soft gel sensor without any skeletal models. 

Skeletal models sometimes increase the durability of a sensor, but the structure itself restricts the sensing range, which requires the sensor to pick up on specific orientations. However, if a sensor does not have a skeletal structure, the manipulation can be achieved without any limitation. 

\subsection{Force Estimation on Hyperelastic Material with Large Deformation }

 For a clear silicone, a material mostly used in vision-based soft tactile sensors, linear elastic models do not accurately describe material behavior. Furthermore, a non-linear elastic model with large deformation requires a precise Finite Element Method (FEM) model with accurate boundary conditions. Some vision-based tactile sensors solved this problem with an inverse FEM model \cite{Ma2019}, expressing marker, or by developing a skeletal structure for precise estimation via image input \cite{sun_soft_2022}.  
However, the sensing range restricted by the either small depth range with planar surface or skeletal structure. DenseTact 2.0 is able to leverage the configuration of hyperelastic material with large deformation on 3D-shaped gel by data-driven approach for the cauchy-elastic material. In other words, our sensor estimates the shape and force with the notion of incompressibility of hyperelastic material. 

\input{table_related_works}

\subsubsection{Rationale of using a Randomized Pattern }

One of the advantages of vision-based tactile sensors is having deflected image information with high resolution. The single image contains rich information on the surface normal, the deflected view of the contact area, and even the force distribution of the image. When the shape of the sensor doesn't have constraints such as the lambertian-surface assumption or a skeletal structure \cite{taylor2021gelslim3, sun_soft_2022}, the modeling for both 3D geometry and force distribution without approximation requires a huge computational load because of the nonlinearity of hyper-elastic materials. The data-driven approach for estimating 3D geometry and force is one way to solve the issue. A data-driven approach requires as many features as possible from a single image. Estimating force from the surface deformation of a vision-based tactile sensor requires a clear signal of the deflected part. Most of the sensors utilize an array of markers for capturing both the shape estimation or estimating wrench information of a specific point. However, the marker-based approach intrinsically has a problem with aliasing. When the sensor is confronted with large deflection, the array of markers or patterns interfere with each other, which increases the error of the force estimation. Therefore, we proposed the randomized pattern surface to imbue the sensor with continuous deflecting information. 


The paper is organized as follows: related work is discussed in \textcolor{red}{Sec. \ref{sec:related_works}}, Sec. \ref{sec:sensor_design} presents the sensor design of DenseTact 2.0, Sec. \ref{sec:shape_force_estimation} presents the method of estimating force and shape with modeling, Sec. \ref{sec:results} shows results for the shape reconstruction model and force estimation model, and the conclusion and future work is discussed in Sec. \ref{sec:conclusion}. 



% \edits{
% Beyond the 3D-shape sensor design with low-construction cost and high sensing resolution, our major contributions include: 
% \begin{inparaenum}[1)]
%     \item \textbf{established a novel and dense calibration process for a model which performs 3D shape reconstruction from a single image with high resolution},  
%     \item \textbf{developed the best neural network for estimating the sensor surface and force vector from the entire sensor by comparing network structures from various models}, 
%     \item developed new models that fit to the position and force sensing with transfer learning, and
%     \item generated a force estimation model from super-soft gel movement with a printed randomized pattern.
    
% \end{inparaenum}
% }

% 




% \section{Related Works}
% \label{sec:related_works}


% The ability for robots to perform complex dexterous manipulation is inherently dependent on the quality of the tactile sensors. The tactile sensor's resolution, noise, bias, and repeatability all contribute directly to the robot's ability to perform robust object manipulation and control. A variety of tactile sensors have been developed with many different approaches including piezoelectric \cite{wettels2009multi}, optics \cite{Dong2017}, resistance \cite{cheng2009flexible}, or capacity \cite{Huh2020}. 
% Recently, vision-based tactile sensors have become very popular compared to previous sensors due to their higher resolution. Optical sensors have proven valuable for tactile sensing with usefulness in detecting both shear and normal forces \cite{Ma2019}, controlling grasping motion \cite{doi:10.1177/02783649211027233}, or adjusting grasp \cite{Hogan2018}. Table \ref{table:comparison} compares vision-based sensor design shapes, resolutions, and calibration methodologies with the proposed sensor of this work in the final row.

% This paper presents a new compact sensor utilizing transfer learning method 



  \begin{figure}[t!]
  
    \vspace{0.2cm}
      \centering
      \includegraphics[width = 3.3 in]{figures/explodedview.png}
    %   \missingfigure[]{content of figure}
      \caption{ \textbf{DenseTact Design}. Exploded view of DenseTact 2.0. The gel mount reflects the light from LED while the gel is covered with the pattern and reflective surface. }
      \label{fig:CAD}
      \vspace{-0.6cm}

  \end{figure}

